Cross-layer Optimization for High Speed Adders: A Pareto Driven Machine Learning Approach

In spite of maturity to the modern electronic design automation (EDA) tools, optimized designs at architectural stage may become sub-optimal after going through physical design flow. Adder design has been such a long studied fundamental problem in VLSI industry yet designers cannot achieve optimal solutions by running EDA tools on the set of available prefix adder architectures. In this paper, we enhance a state-of-the-art prefix adder synthesis algorithm to obtain a much wider solution space in architectural domain. On top of that, a machine learning-based design space exploration methodology is applied to predict the Pareto frontier of the adders in physical domain, which is infeasible by exhaustively running EDA tools for innumerable architectural solutions. Considering the high cost of obtaining the true values for learning, an active learning algorithm is utilized to select the representative data during learning process, which uses less labeled data while achieving better quality of Pareto frontier. Experimental results demonstrate that our framework can achieve Pareto frontier of high quality over a wide design space, bridging the gap between architectural and physical designs.

==> pgfplot/AD.tex <==
% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{10,89,176}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7





\pgfplotsset{
	width =0.35\textwidth,
	height=0.3\textwidth
}
\begin{tikzpicture}[scale=1]
\begin{axis}[
%title=tns vs. area,
xmin=0.33, xmax=0.42,
ymin=1700, ymax=2250,
x label style={at={(axis description cs:0.5,-0.08)}},
y label style={at={(axis description cs:-0.16,.5)}},
xlabel={Critical Delay (ns)},
ylabel={Area ($\mu$m$^2$)},
legend style={
	%at={(0.50,1.30)},
	anchor=north,
	legend columns=1,
	legend pos = north east
}
]

\addplot[blue, style={line width=1.0pt, draw=mygreen}] table {area_delay_pareto_3k.dat};
\addplot[blue, style={line width=1.0pt, draw=mylight}] table {area_delay_pareto.dat};
\addplot[myblue, only marks, mark size=0.3] table {pgfplot/data/8-9/area_delay.dat};
\legend{Real PF, Predicted PF}
\end{axis}
\end{tikzpicture}

==> pgfplot/AT.tex <==
% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{10,89,176}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7





\pgfplotsset{
	width =0.35\textwidth,
	height=0.3\textwidth
}
\noindent
\begin{tikzpicture}[scale=1]
\begin{axis}[
%title=tns vs. area,
xmin=-15, xmax=-12,
ymin=1700, ymax=2350,
x label style={at={(axis description cs:0.5,-0.08)}},
y label style={at={(axis description cs:-0.16,.5)}},
xlabel={TNS (ns)},
ylabel={Area ($\mu$m$^2$)},
legend style={
	%at={(0.50,1.30)},
	%font=\tiny,
	anchor=north,
	legend columns=1,
	legend pos = north east
}
]

\addplot[blue, style={line width=1.0pt, draw=mygreen}] table {area_tns_pareto_3k.dat};
\addplot[blue, style={line width=1.0pt, draw=mylight}] table {area_tns_pareto.dat};
\addplot[myblue, only marks, mark size=0.3] table {pgfplot/data/8-9/area_tns.dat};
\legend{Real PF, Predicted PF}
\end{axis}
\end{tikzpicture}

==> pgfplot/PD.tex <==
% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{10,89,176}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7





\pgfplotsset{
	width =0.35\textwidth,
	height=0.3\textwidth
}
\begin{tikzpicture}[scale=1]
\begin{axis}[
%title=tns vs. area,
xmin=0.33, xmax=0.42,
ymin=5800, ymax=8000,
x label style={at={(axis description cs:0.5,-0.08)}},
y label style={at={(axis description cs:-0.16,.5)}},
xlabel={Critical Delay (ns)},
ylabel={Power ($\mu$w)},
legend style={
	%at={(0.50,1.30)},
	anchor=north,
	legend columns=1,
	legend pos = north east
}
]

\addplot[blue, style={line width=1.0pt, draw=mygreen}] table {power_delay_pareto_3k.dat};
\addplot[blue, style={line width=1.0pt, draw=mylight}] table {power_delay_pareto.dat};
\addplot[myblue, only marks, mark size=0.3] table {pgfplot/data/8-9/power_delay.dat};
\legend{Real PF, Predicted PF}
\end{axis}
\end{tikzpicture}

==> pgfplot/PT.tex <==
% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{10,89,176}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7





\pgfplotsset{
	width =0.35\textwidth,
	height=0.3\textwidth
}
\noindent
\begin{tikzpicture}[scale=1]
\begin{axis}[
%title=tns vs. area,
xmin=-15, xmax=-12,
ymin=5800, ymax=8000,
x label style={at={(axis description cs:0.5,-0.08)}},
y label style={at={(axis description cs:-0.16,.5)}},
xlabel={TNS (ns)},
ylabel={Area ($\mu$w)},
legend style={
	%at={(0.50,1.30)},
	anchor=north,
	legend columns=1,
	legend pos = north east
}
]

\addplot[blue, style={line width=1.0pt, draw=mygreen}] table {power_tns_pareto_3k.dat};
\addplot[blue, style={line width=1.0pt, draw=mylight}] table {power_tns_pareto.dat};
\addplot[myblue, only marks, mark size=0.3] table {pgfplot/data/8-9/power_tns.dat};
\legend{Real PF, Predicted PF}
\end{axis}
\end{tikzpicture}

==> pgfplot/pareto.tex <==

\iffalse
\begin{tikzpicture}
\begin{axis}[
    %title=tns vs. power,
    xmin=-15, ymax=-13,
    ymin=5800, ymax=7400,
    xlabel={TNS},
    ylabel={power},
]
\addplot[red, only marks] table {power_tns.dat};
\addplot[blue] table {power_tns_pareto.dat};
\end{axis}
\end{tikzpicture}
\fi


